$\scriptstyle{BASALT}$: A Rock-Solid Foundation for Epidemic Consensus Algorithms in Very Large, Very Open Networks

Recent works have proposed new Byzantine consensus algorithms for blockchains based on epidemics, a design which enables highly scalable performance at a low cost. These methods however critically depend on a secure random peer sampling service: a service that provides a stream of random network nodes where no attacking entity can become over-represented. To ensure this security property, current epidemic platforms use a Proof-of-Stake system to select peer samples. However such a system limits the openness of the system as only nodes with significant stake can participate in the consensus, leading to an oligopoly situation. Moreover, this design introduces a complex interdependency between the consensus algorithm and the cryptocurrency built upon it. In this paper, we propose a radically different security design for the peer sampling service, based on the distribution of IP addresses to prevent Sybil attacks. We propose a new algorithm, $\scriptstyle{BASALT}$, that implements our design using a stubborn chaotic search to counter attackers' attempts at becoming over-represented. We show in theory and using Monte Carlo simulations that $\scriptstyle{BASALT}$ provides samples which are extremely close to the optimal distribution even in adversarial scenarios such as tentative Eclipse attacks. Live experiments on a production cryptocurrency platform confirm that the samples obtained using $\scriptstyle{BASALT}$ are equitably distributed amongst nodes, allowing for a system which is both open and where no single entity can gain excessive power.

==> algo_consensus.tex <==
\begin{algorithm}[h]
\SetFuncSty{textsf}
\SetKwBlock{Initialization}{initialization}{end}
\SetKwBlock{Function}{function}{end}
\SetKwBlock{OnReceive}{on receive}{end}
\SetKwBlock{Every}{every}{end}
\SetKwData{State}{state}
\SetKwData{Fanout}{fanout}
\SetKw{Send}{Send}
\SetKw{Pull}{Pull}
\SetKw{Push}{Push}
\SetKw{From}{from}
\SetKw{Sample}{Sample}
\SetKw{Wait}{wait until}
\SetKw{Decide}{decide}
\SetKw{Undecided}{undecided}
\SetKwFunction{UpdateSample}{updateSample}
\SetKwFunction{SelectPeer}{selectPeer}
\DontPrintSemicolon

$k \gets $\emph{algorithm parameter: sample size}\\
$\alpha, \beta \gets $\emph{algorithm parameters: sample thresholds}\\
	$\theta \gets $\emph{algorithm parameter: decision threshold}\\

$x \gets $\emph{proposed value}\\
$c \gets 0$;
$S \gets \emptyset$;
$P \gets \emptyset$;
$R \gets \emptyset$\\\vspace{.7em}
\While{\Undecided}{
	\Wait $|S| > k$\\
	$P \gets S$;
	$R \gets \emptyset$;
	$S \gets \emptyset$\\
	\For{$p \in P$}{
		\Send \Pull \KwTo $p$\\
	}
	\Wait $|R| > \alpha k$ \textbf{or until timeout}\\
	\If{$|R| > \alpha k$\label{line:ac_skip_consensus}}{
		\If{$\exists x^*$ s.t. $|\left\{\langle p,x'\rangle \in R, x'=x^*\right\}|>\beta |R|$ \label{line:ac_strong_majority}}{
			\If{$x = x^*$}{
				$c \gets c + 1$ \label{line:ac_gain_confidence}\\
				\lIf{$c \geq \theta$}{\Decide $x$} \label{line:ac_decide}
			}\Else{
				$c \gets c - 1$ \label{line:ac_lose_confidence}\\
				\lIf{$c = 0$}{$x \gets x^*$ \label{line:ac_change_opinion}}
			}
		}
	}
}\vspace{.7em}
\OnReceive(\Sample $p$ \From RPS){
	$S \gets S \cup \{p\}$
}
\OnReceive(\Pull \From $p$){
	\Send \Push $v$ \KwTo $p$
}
\OnReceive(\Push $v'$ \From $p$){
	\lIf{$p \in P$}{
		$R \gets R \cup \{\langle p, v' \rangle\}$
	}
}
\caption{Byzantine-tolerant Binary Consensus using Random Peer Sampling}
\label{alg:consensus}
\end{algorithm}

